Algorithmic transformation of multi-loop Feynman integrals to a canonical basis

The evaluation of multi-loop Feynman integrals is one of the main challenges in the computation of precise theoretical predictions for the cross sections measured at the LHC. In recent years, the method of differential equations has proven to be a powerful tool for the computation of Feynman integrals. It has been observed that the differential equation of Feynman integrals can in many instances be transformed into a so-called canonical form, which significantly simplifies its integration in terms of iterated integrals. The main result of this thesis is an algorithm to compute rational transformations of differential equations of Feynman integrals into a canonical form. Apart from requiring the existence of such a rational transformation, the algorithm needs no further assumptions about the differential equation. In particular, it is applicable to problems depending on multiple kinematic variables and also allows for a rational dependence on the dimensional regulator. First, the transformation law is expanded in the dimensional regulator to derive differential equations for the coefficients of the transformation. Using an ansatz in terms of rational functions, these differential equations are then solved to determine the transformation. This thesis also presents an implementation of the algorithm in the Mathematica package CANONICA, which is the first publicly available program to compute transformations to a canonical form for differential equations depending on multiple variables. The main functionality and its usage are illustrated with some simple examples. Furthermore, the package is applied to state-of-the-art integral topologies appearing in recent multi-loop calculations. These topologies depend on up to three variables and include previously unknown topologies contributing to higher-order corrections to the cross section of single top-quark production at the LHC.

==> dedication.tex <==
\cleardoublepage

\null\vfill\itshape

\begin{flushright}
	Ich widme diese Arbeit \\
	meiner Familie und meinen Freunden
\end{flushright}
\thispagestyle{empty}
\upshape\cleardoublepage



==> epigraph.tex <==
\thispagestyle{empty}
\epigraph{Wir m\"ussen wissen, und wir werden wissen.}{David Hilbert}


==> examples/DrellYanOneMass/DrellYanOneMass.tex <==
\vec{g}^{\,\textup{DYOM}}(\epsilon,s,t)\,\,\,=&\big(I_\textup{DYOM}(0,0,1,1,0,1,0,0,0),&I_\textup{DYOM}(1,0,1,1,0,1,0,0,0),\\
&I_\textup{DYOMx124}(1,0,0,1,0,0,1,0,0),&I_\textup{DYOM}(1,0,0,1,0,0,1,0,0),\\
&I_\textup{DYOM}(0,0,1,1,0,0,1,0,0),&I_\textup{DYOM}(1,0,1,1,0,0,1,0,0),\\
&I_\textup{DYOM}(1,0,1,0,1,0,1,0,0),&I_\textup{DYOM}(0,1,1,0,1,0,1,0,0),\\
&I_\textup{DYOM}(1,1,1,0,1,0,1,0,0),&I_\textup{DYOM}(1,1,0,1,1,0,1,0,0),\\
&I_\textup{DYOM}(1,0,1,1,1,0,1,0,0),&I_\textup{DYOM}(0,1,1,1,1,0,1,0,0),\\
&I_\textup{DYOM}(1,1,1,1,1,0,1,0,0),&I_\textup{DYOM}(0,0,1,0,0,1,1,0,0),\\
&I_\textup{DYOM}(-1,0,1,0,0,1,1,0,0),&I_\textup{DYOM}(0,1,0,1,0,1,1,0,0),\\
&I_\textup{DYOM}(0,1,1,1,0,1,1,0,0),&I_\textup{DYOM}(-1,1,1,1,0,1,1,0,0),\\
&I_\textup{DYOM}(0,1,1,0,1,1,1,0,0),&I_\textup{DYOM}(-1,1,1,0,1,1,1,0,0),\\
&I_\textup{DYOM}(0,1,0,1,1,1,1,0,0),&I_\textup{DYOM}(0,1,1,1,1,1,1,0,0),\\
&I_\textup{DYOM}(-1,1,1,1,1,1,1,0,0),&I_\textup{DYOM}(1,1,1,1,1,1,1,0,0),\\
&I_\textup{DYOM}(1,1,1,1,1,1,1,-1,0)\big).&

==> examples/K4Integral/K4Int1.tex <==
\begin{align}
f^\textup{K4}_{1}=&
\left(1\right)f^{\textup{K4}\prime}_{1},\nonumber\\
\end{align}

==> examples/K4Integral/K4Int2.tex <==
\begin{align}
f^\textup{K4}_{2}=&
\left((x+1)^2\right)f^{\textup{K4}\prime}_{2},\nonumber\\
\end{align}

==> examples/K4Integral/K4Int3.tex <==
\begin{align}
f^\textup{K4}_{3}=&
\left(x^2\right)f^{\textup{K4}\prime}_{3},\nonumber\\
\end{align}

==> examples/K4Integral/K4Int4.tex <==
\begin{align}
f^\textup{K4}_{4}=&
\left(\frac{(2\epsilon-1) (4\epsilon-1) \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right)}{9\epsilon^4}\right)f^{\textup{K4}\prime}_{4},\nonumber\\
\end{align}

==> examples/K4Integral/K4Int5.tex <==
\begin{align}
f^\textup{K4}_{5}=&
\left(\frac{(2\epsilon-1) (4\epsilon-1) \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right)}{9\epsilon^4 (x+1)}\right)f^{\textup{K4}\prime}_{5},\nonumber\\
\end{align}

==> examples/K4Integral/K4Int8.tex <==
\begin{align}
f^\textup{K4}_{8}=&
\left(-\frac{(3\epsilon-2) (4\epsilon-3) \left(\epsilon^5 (288 x+50)-6\epsilon^4 (72 x+5)+\epsilon^3 (262 x+4)-83\epsilon^2 x+14\epsilon x-x\right)}{2\epsilon^3 (2\epsilon-1)^2 (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{1}\nonumber\\
&+\left(\frac{(3\epsilon-2) (4\epsilon-3) \left(84\epsilon^4-40\epsilon^3-8\epsilon^2+7\epsilon-1\right) x}{2\epsilon^3 (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{2}\nonumber\\
&+\left(-\frac{(3\epsilon-2) (3\epsilon-1) (4\epsilon-3) \left(\epsilon^2 (11 x+12)-3\epsilon (2 x+1)+x\right)}{2\epsilon^3 (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{3}\nonumber\\
&+\left(\frac{4 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) x (\epsilon (4 x+3)-x-1)}{9\epsilon (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{4}\nonumber\\
&+\left(-\frac{4 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) x (\epsilon (x-3)+1)}{9\epsilon (2\epsilon-1) (5\epsilon-2) (5\epsilon-1) (x+1)}\right)f^{\textup{K4}\prime}_{5}\nonumber\\
&+\left(-\frac{4 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) (x+2)}{9 (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{6}
+\left(\frac{4 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) \left(2\epsilon^2 (x-4)+6\epsilon-1\right)}{9\epsilon^2 (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{7}
+\left(\frac{4 (3-8\epsilon) \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) x}{9\epsilon (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{8}
+\left(\frac{4 (4\epsilon-1) \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) (x+2)}{9\epsilon^2 (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{9}
+\left(\frac{4 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) \left(2\epsilon^3 (7 x+124)-62\epsilon^2 (x+3)+\epsilon (22 x+31)-x\right)}{9\epsilon^3 (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{10},
\end{align}

==> examples/K4Integral/K4Int9.tex <==
\begin{align}
f^\textup{K4}_{9}=&
\left(-\frac{(3\epsilon-2) (4\epsilon-3) \left(12\epsilon^2-7\epsilon+1\right) \left(4\epsilon^2 (3 x-2)-\epsilon (5 x+1)+x+1\right)}{4\epsilon^3 (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{1}\nonumber\\
&+\left(\frac{(3\epsilon-2) (4\epsilon-3) \left(4\epsilon^5 (31 x-68)+4\epsilon^4 (x+124)-\epsilon^3 (100 x+319)+\epsilon^2 (55 x+97)-3\epsilon (4 x+5)+x+1\right)}{4\epsilon^3 (2\epsilon-1)^2 (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{2}
+\left(-\frac{(3\epsilon-2) (3\epsilon-1) (4\epsilon-3) \left(\epsilon^2 (11 x+18)-\epsilon (6 x+7)+x+1\right)}{4\epsilon^3 (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{3}
+\left(\frac{2 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) \left(\epsilon \left(4 x^2+x-1\right)-x (x+1)\right)}{9\epsilon (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{4}
+\left(-\frac{2 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) \left(\epsilon \left(x^2-6 x+1\right)+2 x\right)}{9\epsilon (2\epsilon-1) (5\epsilon-2) (5\epsilon-1) (x+1)}\right)f^{\textup{K4}\prime}_{5}
+\left(-\frac{2 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) \left(\epsilon \left(x^2-x-4\right)+x+1\right)}{9\epsilon (2\epsilon-1) (5\epsilon-2) (5\epsilon-1) x}\right)f^{\textup{K4}\prime}_{6}
+\left(\frac{2 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) \left(2\epsilon^2 (x-8)+9\epsilon-1\right)}{9\epsilon^2 (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{7}
+\left(-\frac{2 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) \left(2\epsilon^2 (8 x-1)-9\epsilon x+x\right)}{9\epsilon^2 (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{8}
+\left(\frac{2 (7\epsilon-1) \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right)}{9\epsilon^2 (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{9}
+\left(-\frac{2 \left(36\epsilon^3-63\epsilon^2+35\epsilon-6\right) \left(\epsilon^3 (218 x-262)-2\epsilon^2 (56 x-79)+\epsilon (7 x-23)+x+1\right)}{9\epsilon^3 (2\epsilon-1) (5\epsilon-2) (5\epsilon-1)}\right)f^{\textup{K4}\prime}_{10},
\end{align}

==> examples/K4Integral/K4IntegralMIs.tex <==
\vec{g}^{\,\textup{K4}}(\epsilon,s,t)\,\,\,=&\big(I_\textup{K4x124}(1,1,1,1,0,0,0,0,0,0,0,0,0,0,0),&I_\textup{K4x1234}(1,1,1,1,0,0,0,0,0,0,0,0,0,0,0),\\
&I_\textup{K4}(1,1,1,1,0,0,0,0,0,0,0,0,0,0,0),&I_\textup{K4}(2,1,1,1,1,1,0,0,0,0,0,0,0,0,0),\\
&I_\textup{K4}(1,1,2,1,1,1,0,0,0,0,0,0,0,0,0),&I_\textup{K4}(1,1,1,1,2,1,0,0,0,0,0,0,0,0,0),\\
&I_\textup{K4}(1,1,1,1,1,1,-1,0,0,0,0,0,0,0,0),&I_\textup{K4}(1,1,1,1,1,1,0,0,0,0,-1,0,0,0,0),\\
&I_\textup{K4}(1,1,1,1,1,1,0,0,0,0,0,-1,0,0,0),&I_\textup{K4}(1,1,1,1,1,1,0,0,0,0,0,0,0,0,0)\big).

==> examples/MasslessDoubleBox/DBPInt1.tex <==
\begin{align}
f^\textup{DBP}_{1}=&
\left(1\right)f^{\textup{DBP}\prime}_{1}.\nonumber\\
\end{align}

==> examples/MasslessDoubleBox/DBPInt2.tex <==
\begin{align}
f^\textup{DBP}_{2}=&
\left(\frac{2\epsilon (2\epsilon-1)}{(3\epsilon-2) (3\epsilon-1)}\right)f^{\textup{DBP}\prime}_{2}.\nonumber\\
\end{align}

==> examples/MasslessDoubleBox/DBPInt3.tex <==
\begin{align}
f^\textup{DBP}_{3}=&
\left(\frac{2\epsilon (2\epsilon-1) x}{(3\epsilon-2) (3\epsilon-1)}\right)f^{\textup{DBP}\prime}_{1}
+\left(\frac{2\epsilon (2\epsilon-1) x}{(3\epsilon-2) (3\epsilon-1)}\right)f^{\textup{DBP}\prime}_{3},\nonumber
\end{align}


==> examples/MasslessDoubleBox/DBPInt4.tex <==
\begin{align}
f^\textup{DBP}_{4}=&
\left(\frac{2-4\epsilon}{1-3\epsilon}\right)f^{\textup{DBP}\prime}_{4}.\nonumber\\
\end{align}

==> examples/MasslessDoubleBox/DBPInt5.tex <==
\begin{align}
f^\textup{DBP}_{5}=&
\left(\frac{2\epsilon-1}{\epsilon x}\right)f^{\textup{DBP}\prime}_{5}.\nonumber\\
\end{align}

==> examples/MasslessDoubleBox/DBPInt6.tex <==
\begin{align}
f^\textup{DBP}_{6}=&
\left(\frac{(1-2\epsilon)^2}{\epsilon^2 (x+1)}\right)f^{\textup{DBP}\prime}_{6}.\nonumber\\
\end{align}

==> examples/MasslessDoubleBox/DBPInt7.tex <==
\begin{align}
f^\textup{DBP}_{7}=&
\left(\frac{(1-2\epsilon)^2}{\epsilon^2 x^2}\right)f^{\textup{DBP}\prime}_{7}.\nonumber\\
\end{align}

==> examples/MasslessDoubleBox/DBPInt8.tex <==
\begin{align}
f^\textup{DBP}_{8}=&
\left(\frac{(1-2\epsilon)^2}{\epsilon^2 x^2}\right)f^{\textup{DBP}\prime}_{8}.\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/DBNPInt1.tex <==
\begin{align}
f^\textup{DBNP}_{1}=&
\left(\frac{2\epsilon^3 x}{(2\epsilon-1) (3\epsilon-2) (3\epsilon-1)}\right)f^{\textup{DBNP}\prime}_{1}.\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/DBNPInt10.tex <==
\begin{align}
f^\textup{DBNP}_{10}=&
\left(\frac{1}{x^2}\right)f^{\textup{DBNP}\prime}_{10},\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/DBNPInt2.tex <==
\begin{align}
f^\textup{DBNP}_{2}=&
\left(\frac{2\epsilon^3}{(2\epsilon-1) (3\epsilon-2) (3\epsilon-1)}\right)f^{\textup{DBNP}\prime}_{2},\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/DBNPInt3.tex <==
\begin{align}
f^\textup{DBNP}_{3}=&
\left(\frac{2\epsilon^3 (x+1)}{(2\epsilon-1) (3\epsilon-2) (3\epsilon-1)}\right)f^{\textup{DBNP}\prime}_{3},\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/DBNPInt4.tex <==
\begin{align}
f^\textup{DBNP}_{4}=&
\left(\frac{1}{x}\right)f^{\textup{DBNP}\prime}_{4},\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/DBNPInt5.tex <==
\begin{align}
f^\textup{DBNP}_{5}=&
\left(\frac{1}{x+1}\right)f^{\textup{DBNP}\prime}_{5},\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/DBNPInt6.tex <==
\begin{align}
f^\textup{DBNP}_{6}=&
\left(1\right)f^{\textup{DBNP}\prime}_{6},\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/DBNPInt7.tex <==
\begin{align}
f^\textup{DBNP}_{7}=&
\left(\frac{2\epsilon^2}{(2\epsilon-1) (3\epsilon-1)}\right)f^{\textup{DBNP}\prime}_{7},\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/DBNPInt8.tex <==
\begin{align}
f^\textup{DBNP}_{8}=&
\left(\frac{\epsilon}{(2\epsilon-1) x}\right)f^{\textup{DBNP}\prime}_{8},\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/DBNPInt9.tex <==
\begin{align}
f^\textup{DBNP}_{9}=&
\left(\frac{\epsilon}{(2\epsilon-1) x}\right)f^{\textup{DBNP}\prime}_{9},\nonumber\\
\end{align}

==> examples/MasslessDoubleBoxNP/MasslessDoubleBoxNPMIs.tex <==
\vec{g}^{\,\textup{DBPNP}}(\epsilon,s,t)\,\,\,=&\big(I_\textup{DBPNPx124}(1,0,1,0,1,0,0,0,0),&I_\textup{DBPNPx12}(1,0,1,0,1,0,0,0,0),\\
&I_\textup{DBNP}(1,0,1,0,1,0,0,0,0),&I_\textup{DBPNPx123}(1,1,1,1,1,0,0,0,0),\\
&I_\textup{DBPNPx12}(1,1,1,1,1,0,0,0,0),&I_\textup{DBNP}(1,1,1,1,1,0,0,0,0),\\
&I_\textup{DBNP}(0,1,1,0,1,1,0,0,0),&I_\textup{DBPNPx12}(1,1,1,0,1,1,0,0,0),\\
&I_\textup{DBNP}(1,1,1,0,1,1,0,0,0),&I_\textup{DBNP}(0,1,1,1,1,1,1,0,0),\\
&I_\textup{DBNP}(1,1,1,1,1,1,1,0,0),&I_\textup{DBNP}(1,1,1,1,1,1,1,-1,0)\big).

==> examples/SingleTopT1/STT1MIs.tex <==
\vec{g}^{\,\textup{t1}}(\epsilon,s,t,m_t^2,m_W^2)\,\,\,=&\big(I_\textup{t1}(0,1,0,1,0,1,0,0,0),&I_\textup{t1}(0,1,0,1,1,1,0,0,0),\\
&I_\textup{t1}(0,0,1,1,1,1,0,0,0),&I_\textup{t1}(0,1,1,1,1,1,0,0,0),\\
&I_\textup{t1}(1,1,0,0,0,0,1,0,0),&I_\textup{t1}(1,1,-1,0,0,0,1,0,0),\\
&I_\textup{t1}(0,1,0,1,0,0,1,0,0),&I_\textup{t1}(-1,1,0,1,0,0,1,0,0),\\
&I_\textup{t1}(0,0,1,1,0,0,1,0,0),&I_\textup{t1}(0,1,1,1,0,0,1,0,0),\\
&I_\textup{t1}(1,1,1,1,0,0,1,0,0),&I_\textup{t1}(1,1,1,1,-1,0,1,0,0),\\
&I_\textup{t1}(1,1,0,0,1,0,1,0,0),&I_\textup{t1}(1,0,1,0,1,0,1,0,0),\\
&I_\textup{t1}(1,1,1,0,1,0,1,0,0),&I_\textup{t1}(1,1,1,-1,1,0,1,0,0),\\
&I_\textup{t1}(0,1,0,0,0,1,1,0,0),&I_\textup{t1}(0,1,0,1,0,1,1,0,0),\\
&I_\textup{t1}(-1,1,0,1,0,1,1,0,0),&I_\textup{t1}(1,1,0,1,0,1,1,0,0),\\
&I_\textup{t1}(1,1,-1,1,0,1,1,0,0),&I_\textup{t1}(0,1,1,1,0,1,1,0,0),\\
&I_\textup{t1}(0,1,0,0,1,1,1,0,0),&I_\textup{t1}(-1,1,0,0,1,1,1,0,0),\\
&I_\textup{t1}(1,1,0,0,1,1,1,0,0),&I_\textup{t1}(1,1,-1,0,1,1,1,0,0),\\
&I_\textup{t1}(0,1,0,1,1,1,1,0,0),&I_\textup{t1}(1,1,0,1,1,1,1,0,0),\\
&I_\textup{t1}(1,1,1,1,1,1,1,0,0),&I_\textup{t1}(1,1,1,1,1,1,1,0,-1),\\
&I_\textup{t1}(1,1,1,1,1,1,1,-1,0)\big).&

==> examples/SingleTopT1/flycheck_STT1Int10.tex <==
\begin{align}
f^\textup{t1}_{10}=&
\left(\frac{\epsilon^2 \left((9\epsilon-3) x^2+x (\epsilon (5-19 z)+5 z-1)+2 z (\epsilon (5 z-1)-z)\right)}{2 (2\epsilon-1)^2 (3\epsilon-1) (x-z)^2}\right)f^{\textup{t1}\prime}_{7}\\
&+\left(\frac{\epsilon^2 \left((9\epsilon-3) x^2+x (-\epsilon (23 z+5)+7 z+1)+2 z (7\epsilon z+\epsilon-2 z)\right)}{(2\epsilon-1)^2 (3\epsilon-1) (x-z)^2}\right)f^{\textup{t1}\prime}_{8}\\
&+\left(\frac{3\epsilon^2 x (\epsilon (5 x-5 z+3)-x+z-1)}{8 (2\epsilon-1)^2 (3\epsilon-1) (x-z)^2}\right)f^{\textup{t1}\prime}_{9}
+\left(-\frac{3\epsilon^2 x (x-z+1)}{(2\epsilon-1)^2 (x-z)^2}\right)f^{\textup{t1}\prime}_{10}\\
\end{align}


==> examples/SingleTopT2/STT2MIs.tex <==
\vec{g}^{\,\textup{t2}}(\epsilon,s,t,m_t^2,m_W^2)\,\,\,=&\big(I_\textup{t2}(1,1,0,0,0,1,0,0,0),&I_\textup{t2x12}(-1,1,0,1,0,1,0,0,0),\\
&I_\textup{t2x12}(0,1,0,1,0,1,0,0,0),&I_\textup{t2}(-1,1,0,1,0,1,0,0,0),\\
&I_\textup{t2}(0,1,0,1,0,1,0,0,0),&I_\textup{t2}(1,0,0,0,1,1,0,0,0),\\
&I_\textup{t2}(1,1,-1,0,1,1,0,0,0),&I_\textup{t2}(1,1,0,0,1,1,0,0,0),\\
&I_\textup{t2x12}(0,1,0,1,1,1,0,0,0),&I_\textup{t2}(0,1,0,1,1,1,0,0,0),\\
&I_\textup{t2x12}(1,1,-1,1,1,1,0,0,0),&I_\textup{t2x12}(1,1,0,1,1,1,0,0,0),\\
&I_\textup{t2}(1,1,-1,1,1,1,0,0,0),&I_\textup{t2}(1,1,0,1,1,1,0,0,0),\\
&I_\textup{t2}(0,0,1,1,1,1,0,0,0),&I_\textup{t2x12}(-1,1,1,1,1,1,0,0,0),\\
&I_\textup{t2x12}(0,1,1,1,1,1,0,0,0),&I_\textup{t2}(-1,1,1,1,1,1,0,0,0),\\
&I_\textup{t2}(0,1,1,1,1,1,0,0,0),&I_\textup{t2}(-1,1,0,1,0,0,1,0,0),\\
&I_\textup{t2}(0,1,-1,1,0,0,1,0,0),&I_\textup{t2}(0,1,1,1,0,0,1,0,0),\\
&I_\textup{t2x12}(1,1,1,1,-1,0,1,0,0),&I_\textup{t2x12}(1,1,1,1,0,0,1,0,0),\\
&I_\textup{t2}(1,1,1,1,-1,0,1,0,0),&I_\textup{t2}(1,1,1,1,0,0,1,0,0),\\
&I_\textup{t2}(1,1,-1,1,0,1,1,0,0),&I_\textup{t2}(1,1,0,1,0,1,1,0,0),\\
&I_\textup{t2}(1,1,1,1,0,1,1,0,0),&I_\textup{t2}(1,1,-1,1,1,1,1,0,0),\\
&I_\textup{t2}(1,1,0,1,1,1,1,0,0),&I_\textup{t2}(1,0,1,1,1,1,1,0,0),\\
&I_\textup{t2}(1,1,1,1,1,1,1,-2,0),&I_\textup{t2}(1,1,1,1,1,1,1,-1,0),\\
&I_\textup{t2}(1,1,1,1,1,1,1,0,0)\big).&

==> examples/Triplebox/TripleboxMIs.tex <==
\vec{g}^{\,\textup{TB}}(\epsilon,s,t)\,\,\,=&\big(I_\textup{TB}(1,1,1,1,1,1,0,0,0,0,0,0,0,0,0),&I_\textup{TB}(0,1,1,0,1,1,0,1,0,0,0,0,0,0,0),\\
&I_\textup{TB}(0,0,1,1,1,1,1,1,0,0,0,0,0,0,0),&I_\textup{TBx124}(0,1,0,0,1,0,0,1,1,0,0,0,0,0,0),\\
&I_\textup{TB}(0,1,0,0,1,0,0,1,1,0,0,0,0,0,0),&I_\textup{TB}(1,0,0,1,1,0,0,1,1,0,0,0,0,0,0),\\
&I_\textup{TB}(1,1,0,0,1,1,0,1,1,0,0,0,0,0,0),&I_\textup{TB}(0,0,0,1,1,0,1,1,1,0,0,0,0,0,0),\\
&I_\textup{TB}(0,0,0,0,1,1,1,1,1,0,0,0,0,0,0),&I_\textup{TB}(0,1,1,0,1,1,1,1,1,0,0,0,0,0,0),\\
&I_\textup{TB}(1,1,0,0,0,0,1,1,1,1,0,0,0,0,0),&I_\textup{TB}(0,1,1,0,0,0,1,1,1,1,0,0,0,0,0),\\
&I_\textup{TB}(-1,0,1,1,0,0,1,1,1,1,0,0,0,0,0),&I_\textup{TB}(0,0,1,1,0,0,1,1,1,1,0,0,0,0,0),\\
&I_\textup{TB}(1,1,1,1,-1,0,1,1,1,1,0,0,0,0,0),&I_\textup{TB}(1,1,1,1,0,0,1,1,1,1,0,0,0,0,0),\\
&I_\textup{TB}(0,1,0,0,1,0,1,1,1,1,0,0,0,0,0),&I_\textup{TB}(1,-1,0,1,1,0,1,1,1,1,0,0,0,0,0),\\
&I_\textup{TB}(1,0,0,1,1,0,1,1,1,1,0,0,0,0,0),&I_\textup{TB}(1,1,-1,1,1,0,1,1,1,1,0,0,0,0,0),\\
&I_\textup{TB}(1,1,0,1,1,0,1,1,1,1,0,0,0,0,0),&I_\textup{TB}(1,1,-1,0,1,1,1,1,1,1,0,0,0,0,0),\\
&I_\textup{TB}(1,1,0,0,1,1,1,1,1,1,0,0,0,0,0),&I_\textup{TB}(1,1,1,1,1,1,1,1,1,1,-1,0,0,0,0),\\
&I_\textup{TB}(1,1,1,1,1,1,1,1,1,1,0,-1,0,0,0),&I_\textup{TB}(1,1,1,1,1,1,1,1,1,1,0,0,0,0,0)\big).

==> examples/VVT1/VVT1MIs.tex <==
\vec{g}^{\,\textup{t1}}(\epsilon,s,t,m_3,m_4)\,\,\,=&\big(I_\textup{t1}(1,1,1,1,0,0,0,0,0),&I_\textup{t1}(1,0,1,1,1,0,0,0,0),\\
&I_\textup{t1}(0,1,1,1,1,0,0,0,0),&I_\textup{t1}(1,1,1,1,1,0,0,0,0),\\
&I_\textup{t1}(0,1,1,0,0,1,0,0,0),&I_\textup{t1}(0,0,1,0,1,1,0,0,0),\\
&I_\textup{t1}(-1,1,1,0,1,1,0,0,0),&I_\textup{t1}(0,1,1,0,1,1,0,0,0),\\
&I_\textup{t1}(0,0,0,1,1,1,0,0,0),&I_\textup{t1}(1,-1,0,1,1,1,0,0,0),\\
&I_\textup{t1}(1,0,0,1,1,1,0,0,0),&I_\textup{t1}(-1,0,1,1,1,1,0,0,0),\\
&I_\textup{t1}(0,0,1,1,1,1,0,0,0),&I_\textup{t1}(1,0,1,1,1,1,0,0,0),\\
&I_\textup{t1}(0,1,1,1,1,1,0,0,0),&I_\textup{t1}(1,1,0,0,0,1,1,0,0),\\
&I_\textup{t1}(0,0,0,0,1,1,1,0,0),&I_\textup{t1}(1,0,0,0,1,1,1,0,0),\\
&I_\textup{t1}(0,1,0,0,1,1,1,0,0),&I_\textup{t1}(1,1,-1,0,1,1,1,0,0),\\
&I_\textup{t1}(1,1,0,0,1,1,1,0,0),&I_\textup{t1}(-1,1,1,0,1,1,1,0,0),\\
&I_\textup{t1}(0,1,1,0,1,1,1,0,0),&I_\textup{t1}(1,-1,0,1,1,1,1,0,0),\\
&I_\textup{t1}(1,0,0,1,1,1,1,0,0),&I_\textup{t1}(0,0,1,1,1,1,1,0,0),\\
&I_\textup{t1}(1,0,1,1,1,1,1,0,0),&I_\textup{t1}(0,1,1,1,1,1,1,0,0),\\
&I_\textup{t1}(1,1,1,1,1,1,1,-1,0),&I_\textup{t1}(1,1,1,1,1,1,1,0,-1),\\
&I_\textup{t1}(1,1,1,1,1,1,1,0,0)\big).&

==> examples/VVT2/VVT2MIs.tex <==
\vec{g}^{\,\textup{t2}}(\epsilon,s,t,m_3,m_4)\,\,\,=&\big(I_\textup{t2}(1,1,1,1,0,0,0,0,0),&I_\textup{t2}(1,0,1,1,1,0,0,0,0),\\
&I_\textup{t2}(0,1,1,0,0,1,0,0,0),&I_\textup{t2}(0,0,1,0,1,1,0,0,0),\\
&I_\textup{t2}(1,0,0,1,1,1,0,0,0),&I_\textup{t2}(0,0,1,1,1,1,0,0,0),\\
&I_\textup{t2}(1,0,1,1,1,1,0,0,0),&I_\textup{t2}(1,1,1,0,0,0,1,0,0),\\
&I_\textup{t2}(1,0,1,0,1,0,1,0,0),&I_\textup{t2}(1,0,0,0,0,1,1,0,0),\\
&I_\textup{t2}(1,1,0,0,0,1,1,0,0),&I_\textup{t2}(0,1,1,0,0,1,1,0,0),\\
&I_\textup{t2}(1,1,1,0,0,1,1,0,0),&I_\textup{t2}(0,0,0,0,1,1,1,0,0),\\
&I_\textup{t2}(1,-1,0,0,1,1,1,0,0),&I_\textup{t2}(1,0,0,0,1,1,1,0,0),\\
&I_\textup{t2}(1,1,0,0,1,1,1,0,0),&I_\textup{t2}(-1,0,1,0,1,1,1,0,0),\\
&I_\textup{t2}(0,0,1,0,1,1,1,0,0),&I_\textup{t2}(1,0,1,0,1,1,1,0,0),\\
&I_\textup{t2}(-1,1,1,0,1,1,1,0,0),&I_\textup{t2}(0,1,1,0,1,1,1,0,0),\\
&I_\textup{t2}(1,1,1,0,1,1,1,0,0),&I_\textup{t2}(1,-1,0,1,1,1,1,0,0),\\
&I_\textup{t2}(1,0,0,1,1,1,1,0,0),&I_\textup{t2}(0,0,1,1,1,1,1,0,0),\\
&I_\textup{t2}(1,0,1,1,1,1,1,0,0),&I_\textup{t2}(1,1,1,1,1,1,1,-1,0),\\
&I_\textup{t2}(1,1,1,1,1,1,1,0,0)\big).&

==> titlepagePREPRINTNR.tex <==
\KOMAoptions{twoside = false}
\makeatletter
\begin{titlepage}

\begin{picture}(0,0)
\put(380,80){HU-EP-18/02}
\end{picture}
\vspace{-43pt}

\begin{spacing}{1}

\newlength{\parindentbak}
  \setlength{\parindentbak}{\parindent}
\newlength{\parskipbak}
  \setlength{\parskipbak}{\parskip}

\setlength{\parindent}{0pt}
\setlength{\parskip}{\baselineskip}

\thispagestyle{empty}

\begin{center}
{\LARGE \textbf{Algorithmic transformation of multi-loop Feynman integrals to a canonical basis}}
\large

\so{DISSERTATION}

zur Erlangung des akademischen Grades

doctor rerum naturalium\\
(Dr. rer. nat.)\\
im Fach Physik\\
Spezialisierung: Theoretische Physik

eingereicht an der\\
Mathematisch-Naturwissenschaftlichen Fakult\"at\\
der Humboldt-Universit\"at zu Berlin


von\\
\textbf{Herrn M.Sc. Christoph Meyer}\\
%(geboren am 30.01.1987 in Northeim)
\end{center}

\vfill

\large
Pr\"asidentin der Humboldt-Universit\"at zu Berlin: \\
Prof. Dr.-Ing. Dr. Sabine Kunst

Dekan der Mathematisch-Naturwissenschaftlichen Fakult\"at:\\
Prof. Dr. Elmar Kulke
\end{spacing}

\large
Gutachter:
\begin{enumerate}
\item Prof. Dr. Peter Uwer
\item Prof. Dr. Dirk Kreimer
\item Prof. Dr. Stefan Weinzierl\\
\end{enumerate}

\begin{spacing}{1}

\textbf{Tag der m\"undlichen Pr\"ufung: 22. Januar 2018}\\

\setlength{\parindent}{\parindentbak}
\setlength{\parskip}{\parskipbak}
\end{spacing}
\end{titlepage}
\makeatother
\KOMAoptions{twoside}
